SPONGE: A generalized eigenproblem for clustering signed networks

We introduce a principled and theoretically sound spectral method for $k$-way clustering in signed graphs, where the affinity measure between nodes takes either positive or negative values. Our approach is motivated by social balance theory, where the task of clustering aims to decompose the network into disjoint groups, such that individuals within the same group are connected by as many positive edges as possible, while individuals from different groups are connected by as many negative edges as possible. Our algorithm relies on a generalized eigenproblem formulation inspired by recent work on constrained clustering. We provide theoretical guarantees for our approach in the setting of a signed stochastic block model, by leveraging tools from matrix perturbation theory and random matrix theory. An extensive set of numerical experiments on both synthetic and real data shows that our approach compares favorably with state-of-the-art methods for signed clustering, especially for large number of clusters and sparse measurement graphs.

==> SSBM_Model_input.tex <==
%-------------------------------------------------------------------------------------------------------
% SSBM !!!!!!!!!! Moved to SPONGE_GE_analysis_input.tex as it is merged with the section there!!!!!!!!
%--------------------------------------------------------------------------------------------------------
%\vspace{-2mm}
\subsection{Signed stochastic block model}  \label{sec:SSBM_model}
%\vspace{-2mm}
%
\iffalse 
OLD TEXT:

\section{Problem setup}

\subsection{A signed stochastic block model (SSBM) for signed networks}

To compare algorithms in an environment with a known ground truth, we use a signed variant of the stochastic block model to generate test networks. The \emph{signed stochastic block model (SSBM)} we used is defined as follows.

We fix four parameters with which to generate graphs:
\begin{itemize}
    \item $n$ - number of nodes in network
    \item $k$ - number of planted communities
    \item $p$ - edge presence probability
    \item $\eta$ - edge sign flip probability
\end{itemize}

To generate a graph, we take $n$ nodes and place them arbitrarily into $k$ equally-sized (up to rounding) clusters. Each edge in the graph is present independently with probability $p$. Initially, edges within communities are given sign $+1$, and edges between communities are given sign $-1$. Then, the sign of each edge is independently flipped with probability $\eta$. Note that the planted communities in SSBM graphs can only be recoverable by signed clustering algorithms if $\eta<0.5$, since otherwise communities have an equal or lower proportion of positive to negative edges than the graph as a whole, and would not constitute a good clustering output.

\fi 
%%%%%%%
%%%%%%%
%%%%%%%


For ease of exposition, we assume $n$ is a multiple of $k$, and partition the vertices of $G$ into 
$k$-equally sized clusters 
% $\calC_1, \dots, \calC_k$. 
$C_1, \dots, C_k$. 
In particular, we assume w.l.o.g 
that 
% $\calC_l = \set{\frac{(l-1)n}{k}+1,\dots,\frac{l n}{k}}$ 
$C_l = \set{\frac{(l-1)n}{k}+1,\dots,\frac{l n}{k}}$ 
for $l=1,\dots,k$. 
%
The graph $G$ follows the Erd\H{o}s-R\'enyi random graph model $G(n,p)$ wherein each edge takes value $+1$ if both its endpoints are contained in the same cluster, and $-1$ otherwise. To model noise, %in the graph, 
we flip the sign of each edge independently with probability $\eta \in [0,1/2)$. 

\begin{remark} % \hspace{-2mm}
Contrary to stochastic block models for unsigned graphs, we do not require the edge probabilities 
of  % vertices 
intra-cluster edges to be different from those of
%those lying % in different
%across 
inter-cluster edges. While this is 
necessary in the unsigned case for detecting the clusters, it is not the case 
for signed networks since the sign of the edge already achieves this purpose implicitly. 
In fact, as one would expect, it is the parameter $\eta$ that is crucial for identifiability, 
which we show % next
formally in our analysis.
\end{remark}


==> tmp_Formulation <==

% \section{Modeling}

\section{SPONGE: a signed generalized eigenproblem formulation}  \label{sec:formulation_SPONGE}

% \section{SPONGE: Signed Positive - Over - Negative Generalized Eigenproblem}

% Description of the optimization problem considered, and its relaxation.

% G -- $\Gp$
%  H -- $\Gn$
\textbf{Notation}: We let G -- $\Gp$ denote the subgraph of positive edges, and H -- $\Gn$ the subgraph of negative edges. 
\noteMC{Decide on this - since in the theory part we use $A^+$ and $A^-$ + rewrite} 

For any cluster $C\subset V$, we consider the following two measures of \textit{badness} to be minimized
\begin{equation}\label{eq:Cut_G}
 \frac{\Cut_G(C,\overline{C})}{\vol_G(C)},
\end{equation}
\begin{equation}\label{eq:Cut_H}
 \Big( \frac{\Cut_H(C,\overline{C})}{\vol_H(C)} \Big)^{-1} = \frac{\vol_H(C)}{\Cut_H(C,\overline{C})}.
\end{equation}
%
Ideally, $C$ should be such that both~\eqref{eq:Cut_G} and~\eqref{eq:Cut_H} are small. To this end, we first consider the following aggregated objective function that  \textit{merges}~\eqref{eq:Cut_G} and~\eqref{eq:Cut_H}, and instead minimize the following objective function
\begin{equation}\label{eq:objective_function}
\min_{C\subset V}\,\, \frac{\Cut_G(C,\overline{C}) + \vol_H(C)}{ \Cut_H(C,\overline{C}) + \vol_G(C) }
\end{equation}
% 
While at first sight this may seem a rather heuristic interpretation, we provide a sounds theoretical justification for our approach later sections.
% 
An extension for the identification a $k$ disjoint clusters $C_1,\hdots,C_k$ of the set of nodes $V$ corresponds to the following discrete optimization problem
\begin{equation}\label{eq:discrete_optimization_problem}
\min_{C_1,\hdots,C_k} \sum_{i=1}^k \frac{\Cut_G(C_i,\overline{C_i}) + \vol_H(C_i)}{\Cut_H(C_i,\overline{C_i}) + \vol_G(C_i)}
\end{equation}
Given a subset $C_i\subset V$ we can define a normalized indicator vector $X_{C_i}$
\begin{equation}
(X_{C_i})_j = 
 \begin{cases} 
1/\sqrt{\Cut_H(C_i,\overline{C_i}) + \vol_G(C_i)} & \text{ if } v_j \in C_i \\
0 & \text{ otherwise } 
\end{cases}
\end{equation}
With this in mind, we can now express the discrete optimization problem~\eqref{eq:discrete_optimization_problem} as follows:
\begin{equation}\label{eq:discrete_optimization_problem-2}
\min_{C_1,\hdots,C_k} \sum_{i=1}^k \frac{ X_{C_i}^T (\Lun_G + \D_H) X_{C_i} }{ X_{C_i}^T (\Lun_H + \D_G) X_{C_i} }
\end{equation}
which is clearly NP hard. A natural way to overcome this limitation goes by dropping the discreteness condition by allowing each vector $X_{C_i}$ to take values in $\mathbb{R}^n$. For this, we introduce a new set of vectors $z_1,\ldots,z_k\in\mathbb{R}^k$ such that they are orthonormal with respect to $\Lun_H+\D_G$, i.e. 
\begin{itemize}
 \item $z_i^T  (\Lun_H+\D_G) z_i =1$, and 
 \item $z_i(\Lun_H+\D_G)z_j= 0$
\end{itemize}
leading to the following modified version of Equations~\eqref{eq:discrete_optimization_problem} and \eqref{eq:discrete_optimization_problem-2}
\begin{equation}\label{eq:discrete_optimization_problem-z}
 \min_{z_i(\Lun_H+\D_G)z_j=\delta_{ij}} \sum_{i=1}^k \frac{ z_i^T (\Lun_G + \D_H) z_i }{ z_i^T (\Lun_H + \D_G) z_i }
\end{equation}
Observe that the above considered orthonormality of vectors $z_1,\ldots,z_k$ with respect to $\Lun_H+\D_G$ leads to a particular eigenvalue problem. Indeed, consider the change of variables 
\begin{equation}
y_i=(\Lun_G+\D_H)^{1/2}z_i  
\end{equation}
Then, orthonormality constraints of Equation~\eqref{eq:discrete_optimization_problem-2}
become $y_i^T y_j = \delta_{ij}$. In fact, by defining the matrix $Y=[y_1,\ldots,y_k ]\in\mathbb{R}^{n\times k}$ we can rephrase Equation~\eqref{eq:discrete_optimization_problem-2} into
%
\begin{equation}
\footnotesize
\label{eq:discrete_optimization_problem-y}
 \min_{Y^T Y = I} \Tr \Big( Y^T (\Lun_H + \D_G)^{-1/2} (\Lun_G+\D_H) (\Lun_H + \D_G)^{-1/2} Y \Big)
\end{equation}
The solution to Equation~\eqref{eq:discrete_optimization_problem-y} are the eigenvectors corresponding to the $k$-smallest eigenvalues of the matrix $(\Lun_H + \D_G)^{-1/2} (\Lun_G+\D_H) (\Lun_H + \D_G)^{-1/2}$. One can also verify that $(\lambda,v)$ is an eigenpair of the previous matrix if and only if $(\lambda, (\Lun_H + \D_G)^{-1/2}v)$ is an eigenpair of $(\Lun_H + \D_G, \Lun_G + \D_H)$. \pedro{verify this: I think its worthwhile putting this as a theorem/lemma. I am not sure if the last statement has the wrong order, i.e. $(\Lun_H + \D_G, \Lun_G + \D_H)$ instead of $(\Lun_G + \D_H, \Lun_H + \D_G)$... does the ordering matter?}.

\begin{lemma}\label{lemma:eigpair-generalizedeigpair}
 $(\lambda,v)$ is an eigenpair of $(\Lun_H + \D_G)^{-1/2} (\Lun_G+\D_H) (\Lun_H + \D_G)^{-1/2}$ if and only if $(\lambda, (\Lun_H + \D_G)^{-1/2}v)$ is an eigenpair of $(\Lun_H + \D_G, \Lun_G + \D_H)$.
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lemma:eigpair-generalizedeigpair}]
Let $A = \Lun_H + \D_G$ and $B = \Lun_G + \D_H$. Then by Lemma~\ref{lemma:aux-1} we can see that
 $(\lambda,v)$ is an eigenpair of $A^{-1/2}BA^{-1/2}$ if and only if 
 $(\lambda, A^{-1/2}v)$ is an eigenpair of $(B,A)$.
\end{proof}



\begin{lemma}\label{lemma:aux-1}
 Let $A,B$ be symmetric positive definite matrices. 
 Then $(\lambda,v)$ is an eigenpair of $A^{-1/2}BA^{-1/2}$ if and only if 
 $(\lambda, A^{-1/2}v)$ is an eigenpair of $(B,A)$.
 \begin{proof}
    \begin{equation*}
    A^{-1/2}BA^{-1/2}v = \lambda v \iff BA^{-1/2}v = \lambda A^{1/2}v \iff Bw = \lambda Aw 
    \end{equation*}
    where $w=A^{-1/2}v$.
    \end{proof}
\end{lemma}


